Competitive Facility Location under Cross-Nested Logit Customer Choice Model: Hardness and Exact Approaches

We study the competitive facility location problem, where a firm aims to establish new facilities in a market already occupied by competitors. In this problem, customer behavior is crucial for making optimal location decisions. We explore a general class of customer choice models, known as the cross-nested logit (CNL) model, which is recognized for its flexibility and generality in predicting people's choice behavior. To explore the problem, we first demonstrate that it is NP-hard, even when there is only one customer class. We further show that this hardness result is tight, as the facility location problem under any simpler choice models (such as the logit or nested logit) is polynomial-time solvable when there is one customer class. To tackle the resulting facility location problem, we demonstrate that the objective function under a general cross-nested structure is not concave. Interestingly, we show that by a change of variables, the objective function can be converted to a convex program (i.e., a maximization problem with a concave objective and convex constraints), enabling it to be solved to optimality via an outer-approximation algorithm. Extensive experiments show the efficiency of our approach and provide analyses on the benefits of using the cross-nested model in the facility location context.

==> include.tex <==
\usepackage[a4paper]{geometry}
\usepackage[main=american]{babel}
\usepackage{array}
\usepackage{float}
%\usepackage{textcomp}
\usepackage{multirow}
%\usepackage{xcolor}
%\usepackage{adjustbox}
%\usepackage{blindtext}
%\usepackage{pifont}
%\usepackage{latexsym}
\usepackage{amsmath,amsfonts,amssymb,nicefrac}
\usepackage{graphicx}
\usepackage{url}
\usepackage{lipsum}
\usepackage[unicode=true, colorlinks=true,linkcolor=blue, citecolor=blue, urlcolor=blue]{hyperref}
\usepackage{subfig}
\usepackage[figuresright]{rotating}
%\usepackage{algorithm}
\usepackage{algpseudocode}
%\usepackage{ulem}
\bibliographystyle{abbrvnat}
\usepackage{algorithmicx}
\usepackage[ruled,vlined]{algorithm2e}

\usepackage[square,sort,comma,numbers]{natbib}
\bibstyle{plainnat}

\AtBeginDocument{\renewcommand*\bibname{References}}

==> sections/1.Introduction.tex <==
\section{Introduction}
\textbf{Notation}: Boldface characters represent matrices or vectors or sets, and $a_i$ denotes the $i$-th element of $\textbf{a}$ if $\textbf{a}$ is indexable. We use $[m]$, for any $m\in N$, to denote the set $\{1, . . . ,m\}$.

==> sections/2.Problem_Formulations.tex <==
\section{Problem Formulations}
\subsection{Additive random utility model}
% % COR 2023, Joint Location and Cost Planning in Maximum Capture Facility Location under Random Utilities
The discrete choice framework assumes that each individual (decision-maker) $t$ associates a utility $U_{ti}$ with each alternative $i$ in a choice set $S_t$. It is then assumed that each utility $U_{ti}$ consists of two parts: a deterministic part $V_{ti}$ that contains some observed attributes of the corresponding alternative and the individual $t$, and a random term $\epsilon_{ti}$ that is unknown to the analyst.

Under the RUM framework, the probability that individual $t$ selects an alternative $i\in S_t$ is equal to the probability of $U_{ti}$ being the largest of all $U_{tj},\:j\in S_t$. This probability can be computed as
\begin{align*}
    P(i|S_t) = P(U_{ti} \geq U_{tj}, \: \forall j\in S_t).
\end{align*}
Given the deterministic parts $V_{tj},\:j\in S_t$, this probability will depend on the assumptions on the distribution of the random terms $\epsilon_{nj},\:j\in S_t$.

Under the additive RUM (ARUM) framework, the deterministic parts and random terms have an additive form, $U_{ti} = V_{ti} + \epsilon_{ti}$. Then, the probability that individual $t$ selects an alternative $i\in S_t$ become:
\begin{align*}
    P(i|S_t) &= P(V_{ti} + \epsilon_{ti} \geq V_{tj} + \epsilon_{tj},\:\forall j\in S_t)
\end{align*}
Using the multinomial logit (MNL) model with assumptions that $\epsilon_{ti}$ are i.i.d and follow the standard Gumbel distribution, then by Gumbel-max trick, the choice probabilities have the following form
\begin{align*}
    P(i|S_t) = P(i = \arg\max_{j} (V_{tj} + \epsilon_{tj})) = \frac{e^{V_{ti}}}{\sum_{j\in S_t}e^{V_{tj}}},\:\forall i\in S_t.
\end{align*}

\subsection{Cross-Nested Logit as an Additive RUM model}
% Follow paper 2002, Structural choice analysis with nested logit models
% 2023, Constrained Assortment Optimization under Cross-Nested Logit
Following the basic idea of the cross-nested logit (CNL) model, there are $N$ subsets (or nests) $C_1,C_2,\ldots,C_N$ of the choice set $S = \bigcup_{t}S_t$ according to their attributes, such as scale, population density, or the proximity to the city center. They may share the same locations and assume that the competitors can belong to any nest.

Under the ARUM CNL-based model, the customer's choice behavior can be decomposed into two stages, each of which takes the form of the standard logit. In the first stage, the customer zone $t\in I$ selects a nest $C_{n}$ from $N$ nests. Each nest $C_{n}$ is thus selected with a probability 
\begin{align*}
    P(C_{n} | S) = \dfrac{W_{tn}^{\sigma_{n}}}{U_t^c + \sum_{n'\in [N]}W_{tn'}^{\sigma_{n'}}} 
\end{align*}
where $\sigma_{n}$ is the dissimilarity parameter of the nest $C_n$ and $W_{tn} = U_{tn}^c + \sum_{i\in C_{n}} e^{V_{ti}/\sigma_{n}}$ is the attractiveness of the nest $C_{n}$, $U_{tn}^c$ is the exponential of the utility when choosing a competitor's facility in the nest $C_{n}$ and $U_t^c$ is the customer zone $t$'s utility when not choosing any facility. %It is typically assumed that the value of $\sigma_{n}$ varies in the unit interval for all nests to guarantee that the model is consistent with the RUM framework. 

In the second stage, the customer $t$ chooses an element from the nest $C_{n}$ selected in the previous stage. In this case, the utilities are rescaled by the inverse of the dissimilarity parameter $\sigma_{n}$ for its nest. So, the conditional choice probability of choosing alternative $i$ given some alternative in its nest $C_{n}$ is chosen is
\begin{align*}
    P(i|C_{n}) = \dfrac{e^{V_{ti}/\sigma_{n}}}{U_{tn}^c + \sum_{i'\in C_{n}}e^{V_{ti}/\sigma_{n}}} 
    = \dfrac{e^{V_{ti}/\sigma_{n}}}{W_{tn}}
\end{align*}
Otherwise, if $i\notin C_{n}$ then $P(i|C_{n}) = 0$.
Then, through the law of total probability, the probability of a customer with choice set $S$ when choosing alternative $i$ can be computed as
\begin{align*}
    P(i|S) 
    = \sum_{n'\in [N]} P(i|C_{n'})P(C_{n'}|S) 
    &= \dfrac{e^{V_{ti}/\sigma_{n}}}{W_{tn}}
     \dfrac{W_{tn}^{\sigma_{n}}}
     {\sum_{n'\in [N]}W_{tn'}^{\sigma_{n'}}}\\
    &= \dfrac{e^{V_{ti}/\sigma_{n}}\cdot W_{tn}^{(\sigma_{n}-1)}}
    {U_t^c + \sum_{n'\in [N]}W_{tn'}^{\sigma_{n'}}}, \quad i\in C_{n}.
\end{align*}
\subsection{Maximum Capture Facility Location Problem}
% COR 2023, Joint Location and Cost Planning in Maximum Capture Facility Location under Random Utilities
In the context of the competitive maximum capture facility location (MCFL) problem, a ``newcomer" ﬁrm aims to locate new facilities in a competitive market where there are existing facilities from a competitor. The ﬁrm’s objective is to maximize the expected captured market share achieved by attracting customers to new facilities. To capture the customers' demand, we suppose that a customer selects a facility according to an ARUM discrete choice model. In this context, each customer $t$ associates each new facility $i$ with a random utility $U_{ti}$, and choices are made by maximizing his/her utilities. The ﬁrm’s decisions are a set of locations to setup new facilities and costs to spend on new facilities. In the following, we describe in detail our problem formulations under ARUM CNL-based models. 

Assume that there are $m$ possible locations to locate new facilities. Let us denote by $S = [m]$ the set of all possible locations and by $I$ the set of all customer zones. Depending on the application, $I$ can be a set of geographical zones where customers are located. Assume that there are $q_{n}$ customers for each zone $t\in I$. Let $V_{ti}$ be the deterministic utility that customer zone $t\in I$ assign to a facility at location $i\in S$ when making choice decisions. The deterministic utility can be measured by distances, costs, availability of parking spaces, etc. 

We assume that the customer's choice behavior comprises two stages following the CNL-based model. Under the ARUM CNL-based model, the MCFL problem can be formulated as
\begin{align*}
    \max_{\textbf{x}}&\left\{
    \mathcal{F}(\textbf{x})=\sum_{t\in I}q_{t}
    \sum_{n\in [N]}\sum_{i\in C_{n}}x_{i}P(i|S)
    \right\} 
    \\ \text{subject to}\quad 
    &\sum_{i\in S}x_i\leq B.\\
    &x_i\in \{0,1\}, \quad \forall i\in S.
\end{align*}

Let $W_{tn} = U_{tn}^c + \sum_{i\in C_{n}} x_{i}e^{V_{ti}/\sigma_n}, \forall t\in I, n\in [N]$, then the objective function of the MCFL problem can be further written as follows
\allowdisplaybreaks
\begin{align*}
    \mathcal{F}(\textbf{x}) 
    &= \sum_{t\in I}q_{t}
    \sum_{n\in [N]}\sum_{i\in C_{n}}x_{i}P(i|S)\\
    &= \sum_{t\in I}q_{t}
    \sum_{n\in [N]}\sum_{i\in C_{n}}x_i\dfrac{e^{V_{ti}/\sigma_n}
    \cdot W_{tn}^{\sigma_{n}-1}}
    {U_t^c + \sum_{n'\in [N]}W_{tn'}^{\sigma_{n'}}}\\
    &= \sum_{t\in I}q_{t}
    \sum_{n\in [N]}\dfrac{W_{tn}^{\sigma_{n}-1}}
    {U_t^c + \sum_{n'\in [N]}W_{tn'}^{\sigma_{n'}}}
    \sum_{i\in C_{n}}x_{i}e^{V_{ti}/\sigma_n}\\
    &= \sum_{t\in I}q_{t}
    \sum_{n\in [N]}\dfrac{W_{tn}^{\sigma_{n}-1}}
    {U_t^c + \sum_{n'\in [N]}W_{tn'}^{\sigma_{n'}}}(W_{tn}-U_{tn}^c)\\
    &= \sum_{t\in I}q_{t}\cdot \dfrac{\sum_{n\in [N]}W_{tn}^{\sigma_{n}}}
    {U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}}} - \sum_{t\in I}q_{t}\cdot \dfrac{\sum_{n\in [N]}W_{tn}^{\sigma_{n}-1}U_{tn}^c}
    {U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}}}\\
    &= \sum_{t\in I}q_{t} - \sum_{t\in I}q_{t}\cdot \dfrac{U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}-1}U_{tn}^c}{U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}}}
\end{align*}
\textit{Show that below formulation is non-concave and if the competitor is not in any nest, it is concave by previous study or proof.}
Then, the cost optimization MCP can be reformulated as
\begin{align}
    \max_{\textbf{x}}&\left\{
    \mathcal{F}(\textbf{x})=\sum_{t\in I}q_{t} - \sum_{t\in I}q_{t}\cdot \dfrac{U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}-1}U_{tn}^c}{U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}}}
    \right\} \label{MCP-Cost:obj}
    \\ \text{subject to}\quad 
    &W_{tn} = U_{tn}^c + \sum_{i\in C_{n}} x_{i}e^{V_{ti}/\sigma_n}, \quad \forall t\in I, n\in [N].\label{MCP-Cost:attractive-ness}\\
    &\sum_{i\in S}x_i\leq B.\label{MCP-Cost:maxCons}\\
    &x_{i}\in \{0,1\}, \forall i\in S. \label{MCP-Cost:domain}
\end{align}

\[
f(x) = \frac{(2x+3)^{-0.3} + (1x+2)^{-0.7}}{2+(2x+3)^{0.7} + (1x+2)^{0.3}} + \frac{(5x+2)^{-0.2} + (2x+2)^{-0.3}}{2+(5x+2)^{0.8} + (2x+2)^{0.7}}
\]

\subsubsection{Facility Location Prolem under Nested logit model is concave}
Consider $\mathcal{F}: [0,1]^m\to \mathcal{R}$, $\mathcal{F}(\text{x}) = \sum_{t\in I}q_{t} - \sum_{t\in I}q_{t}\cdot \dfrac{U_t^c}{U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}}}$

We have $\sigma_n\leq 1$ and $W_{tn}$ is concave, thus $W_{tn}^{\sigma_n}$ is concave.

Now, we have $U_t^c + \sum_{n\in [N]} W_{tn}^{\sigma_n}$ is concave and positive.

Therefore $\dfrac{U_t^c}{U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_n}}$ is convex, leading to $\mathcal{F}(x)$ is concave.
\subsubsection{Facility Location Prolem under Cross-Nested logit model is non-concave}
Assume that $\mathcal{F}(x)$ is concave. Then, we have $\mathcal{G}(x) = \sum_{t\in I}q_{t}\cdot \dfrac{U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}-1}U_{tn}^c}{U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}}}$ is convex.

Using the first-order condition of $\mathcal{G}(x)$, we have
\begin{align*}
    \mathcal{G}(\text{y}) \geq \mathcal{G}(\text{x}) + \nabla\mathcal{G}(\text{x})^T(\text{y}-\text{x})
\end{align*}

Theorem 1. $\mathcal{G}(x)$ is strictly decreasing in every dimension.

From Theorem 1, we have $\mathcal{G}(e) < \mathcal{G}(0)$.

Let $\mathcal{A}_t(x) = U_t^c + \sum_{n\in [N]}W_{tn}(x)^{\sigma_n-1}U_{tn}^c, \mathcal{B}_t(x) = U_t^c + \sum_{n\in [N]}W_{tn}(x)^{\sigma_n},\forall t\in I$.

Then, $\mathcal{A}_t(\text{0}) = \mathcal{B}_t(\text{0}) = U_t^c + \sum_{n\in [N]}(U_{tn}^c)^{\sigma_n}$ and $\mathcal{G}(\text{0}) = \sum_{t\in I}q_t$.

We have,
\begin{align*}
    \sum_{i\in S}\dfrac{\partial A_t}{\partial x_i}(\text{x})(y_i-x_i) &= \sum_{i\in S}\left(\sum_{n\in [N]: i\in C_n}(\sigma_n - 1)(U_{tn}^c + \sum_{i'\in C_n}x_{i'}c_{tni'})^{\sigma_n-2}c_{tni}U_{tn}^c\right)(y_i-x_i)\\
    &= \sum_{n\in [N]}(\sigma_n - 1)U_{tn}^c(U_{tn}^c + \sum_{i\in C_n}x_{i}c_{tni})^{\sigma_n-2}\left(\sum_{i\in C_n}c_{tni}(y_i-x_i)\right)\\
    \sum_{i\in S}\dfrac{\partial B_t}{\partial x_i}(\text{x})(y_i-x_i) &= \sum_{i\in S}\left(\sum_{n\in [N]: i\in C_n}\sigma_{n}(U_{tn}^c + \sum_{i'\in C_n}x_{i'}c_{tni'})^{\sigma_n-1}c_{tni}\right)(y_i-x_i)\\
    &= \sum_{n\in [N]}\sigma_{n}(U_{tn}^c + \sum_{i\in C_n}x_{i}c_{tni})^{\sigma_n-1}\left(\sum_{i\in C_n}c_{tni}(y_i-x_i)\right)
\end{align*}
where $c_{tni} = e^{V_{ti}/\sigma_n},\forall t\in I, n\in [N], i\in S$.

Therefore,
\begin{align*}
    \nabla\mathcal{G}(\text{x})^T(y-x) 
    &= \sum_{i\in S}(y_i-x_i)\sum_{t\in I}q_t\left(\dfrac{\nabla_i\mathcal{A}_t(\text{x})}{\mathcal{B}_t(\text{x})} - \dfrac{\mathcal{A}_t(\text{x})\nabla_i\mathcal{B}_t(\text{x})}{\mathcal{B}_t(\text{x})^2}\right)\\
    &= \sum_{t\in I}q_t\dfrac{
    \mathcal{B}_t(x)\sum_{i\in S}(y_i-x_i)\nabla_i\mathcal{A}_t(x) -
    \mathcal{A}_t(x)\sum_{i\in S}(y_i-x_i)\nabla_{i}\mathcal{B}_t(x)
    }{\mathcal{B}_{t}(x)^2}\\
    &= \sum_{t\in I}\dfrac{q_t}{\mathcal{B}_t(x)^2}
    \sum_{n\in [N]}W_{tn}(x)^{\sigma_n-2}(W_{tn}(y)-W_{tn}(x))\\
    &\qquad \bigg((\sigma_n-1)U_{tn}^c\mathcal{B}_t(x) - \sigma_nW_{tn}(x)\mathcal{A}_t(x)\bigg)
\end{align*}

\begin{align*}
    &\mathcal{G}(\text{x}) + \nabla\mathcal{G}(\text{x})^T(y-x) \\
    &=  \sum_{t\in I}\dfrac{q_t}{\mathcal{B}_t(x)}\left(\mathcal{A}_t(\text{x}) + 
    \dfrac{\sum_{n\in [N]}W_{tn}(x)^{\sigma_n-2}(W_{tn}(y)-W_{tn}(x))((\sigma_n-1)U_{tn}^c\mathcal{B}_t(x) - \sigma_nW_{tn}(x)\mathcal{A}_t(x))}{\mathcal{B}_t(x)}\right)
\end{align*}

==> sections/4.Solution_Method.tex <==
\section{Solution Method}
%approximate based on x or W?
%x -> complex
%W -> constraints?
% Follow the paper KSE 2022, Approximation Methods for a Nonlinear Competitive Facility Cost Optimization Problem
% 2023, Constrained Assortment Optimization under Cross-Nested Logit
\subsection{Cutting Plane Approach}
Let's divide $I$ into $\mathcal{L}$ disjoint groups $\mathcal{D}_1,\mathcal{D}_2,\ldots,\mathcal{D}_{\mathcal{L}}$ such that $\cup_{l\in [\mathcal{L}]}\mathcal{D}_{l} = I$.

Then, the objective function can be written as: $\mathcal{F}(\text{x}) = \sum_{l\in [\mathcal{L}]}F_l(\text{x})$, where
\begin{align*}
    F_l(\text{x}) = \sum_{t\in \mathcal{D}_l}q_{t} - \sum_{t\in \mathcal{D}_l}q_{t}\cdot \dfrac{U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}-1}U_{tn}^c}{U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}}}
\end{align*}
\textit{$F_l(\text{x})$ is monotonically increasing and submodular. Proof? -> refer to a paper by Emma Frejinger.? A model-free approach for solving choice-based competitive facility location problems using simulation and submodularity.}

Then, the cost optimization MCP can be reformulated as
\begin{align}
    \max_{\textbf{x}}&\left\{
    \mathcal{F}(\textbf{x})=\sum_{l\in [\mathcal{L}]}\theta_l
    \right\} \label{MCP-Cost:obj}
    \\ \text{subject to}\quad 
    &\theta_l \leq F_l(\text{x}), \quad \forall l\in [\mathcal{L}]\\
    &\text{Constraints }\eqref{MCP-Cost:attractive-ness}-\eqref{MCP-Cost:maxCons}-\eqref{MCP-Cost:domain}
\end{align}
Let's define $\rho_{li}(\text{x}) = F_l(\text{x} + \textbf{e}_i) - F_l(\text{x})$, where $\textbf{e}_i$ is a binary vetor of size $m$ with zero elements except the $k$-th element and $\text{x}+\textbf{e}_i$ denote the binary vector such that each element of it is the maximum of the corresponding elements in vector $\text{x}$ and $\textbf{e}_i$.

\textit{Submodular cut refer to} \cite{1981-submodular-cut}

Then, for any candidate solution $\text{x}^*$, we have the following linear cuts:
\begin{align}
    \theta_{l} &\leq \sum_{i\in S}\rho_{li}(\text{x}^*)(1-\text{x}^*_i)x_i - \sum_{i\in S}\rho_{li}(\textbf{e}-\textbf{e}_i)\text{x}^*_i(1-x_i) + F_l(\text{x}^*)\\
    \theta_{l} &\leq \sum_{i\in S}\rho_{li}(\textbf{0}) - \sum_{i\in S}\rho_{li}(\text{x}^*-\textbf{e}_i)\text{x}^*_i(1-x_i) + F_l(\text{x}^*)
\end{align}
Let 
\begin{align*}
    r_{tn} &= \ln \left(W_{tn}^{\sigma_{n}-1}U_{tn}^c\right),\forall t\in I, n\in [N]\\
    R_t &= \ln\left(U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}}\right), \forall t\in I.
\end{align*}
Then, 
\begin{align*}
    \widehat{F}_l(\textbf{x, r, R}) = \sum_{t\in \mathcal{D}_l}q_{t} - \sum_{t\in \mathcal{D}_l}q_{t}\left(U_t^c.e^{-R_t} + \sum_{n\in [N]}e^{r_{tn}-R_t}\right)
\end{align*}
Then, the cost optimization MCP formulation can be reformulated as follows
\begin{align}
    \max_{\textbf{z, r, R}}&\quad 
    \sum_{l\in [\mathcal{L}]}\theta_l
    \label{MCP-Cost:obj-conv}\\
    \text{s.t.}\quad 
    &\theta_l \leq \widehat{F}_l(\textbf{x, r, R}), \quad \forall l\in [\mathcal{L}]\\
    &r_{tn} \geq \ln(U_{tn}^c) + (\sigma_n - 1)\ln W_{tn},\quad \forall t\in I, n\in [N].\label{MCP-Appr:cons1}\\
    &e^{R_t} \leq U_t^c + \sum_{n\in [N]}W_{tn}^{\sigma_{n}},\quad \forall t\in I.\label{MCP-Appr:cons2}\\
    &\text{Constraints }\eqref{MCP-Cost:attractive-ness}-\eqref{MCP-Cost:maxCons}-\eqref{MCP-Cost:domain}\label{MCP-cost:other}
\end{align}

Denote that $g^1_{tn} = \ln(U_{tn}^c) + (\sigma_n - 1)\ln W_{tn} - r_{tn}$ and $g^2_{t} = e^{R_t} - U_t^c - \sum_{n\in [N]}W_{tn}^{\sigma_{n}}$. These functions and the objective \eqref{MCP-Cost:obj-conv} are convex so that the cutting plane will return an optimal solution after a finite number of iterations.
\small\begin{align}
    \max_{\text{z, r, R, }\theta}& \quad \sum_{l\in [\mathcal{L}]}\theta_l \label{MCP-Cost:obj-conv-cutting}\\
    \text{s.t.}\quad 
    &\theta_{l} \leq \sum_{i\in S}\rho_{li}(\text{x}^*)(1-\text{x}^*_i)x_i - \sum_{i\in S}\rho_{li}(\textbf{e}-\textbf{e}_i)\text{x}^*_i(1-x_i) + F_l(\text{x}^*), \quad \forall l\in [\mathcal{L}]\label{MCP-Cost:submodular1}\\
    &\theta_{l} \leq \sum_{i\in S}\rho_{li}(\textbf{0})(1-\text{x}^*_i)x_i- \sum_{i\in S}\rho_{li}(\text{x}^*-\textbf{e}_i)\text{x}^*_i(1-x_i) + F_l(\text{x}^*), \quad \forall l\in [\mathcal{L}]\label{MCP-Cost:submodular2}\\
    &\theta_l \leq \widehat{F}_l(\text{x*, r*, R*}) + \nabla \widehat{F}_l(\text{x*, r*, R*})\begin{pmatrix}
        \text{x}-\text{x}^*\\\text{r}-\text{r*}\\\text{R}-\text{R*}
    \end{pmatrix}, \quad \forall l\in [\mathcal{L}]\label{sub-MCP-Cost:cut-obj}\\
    &g^1_{tn}(\text{x*,r*}) + \nabla g^1_{tn}(\text{x*,r*})\begin{pmatrix}
        \text{x}-\text{x}^*\\\text{r}-\text{r*}
    \end{pmatrix} \leq 0,\quad \forall t\in I, n\in [N]\label{sub-MCP-Cost:cut-cons1}\\
    &g^2_{t}(\text{x*,R*}) + \nabla g^2_{t}(\text{x*,R*})\begin{pmatrix}
        \text{x}-\text{x}^*\\\text{R}-\text{R*}
    \end{pmatrix} \leq 0,\quad \forall t\in I\label{sub-MCP-Cost:cut-cons2}\\
    &\text{Constraints }\eqref{MCP-Cost:attractive-ness}-\eqref{MCP-Cost:maxCons}-\eqref{MCP-Cost:domain}\label{sub-MCP:other}
\end{align}

\begin{algorithm}[H]              %new code
        \caption{Cutting Plane Approach}
        \DontPrintSemicolon
        Choose a small $\epsilon \geq 0$ as the optimal gap.\;
         Initialize the master problem (Sub-MCP) \eqref{MCP-Cost:obj-conv-cutting} - \eqref{sub-MCP:other}.\;
         \KwIn{\text{z*, r*, R*} satisfy \eqref{MCP-Appr:cons1} - \eqref{MCP-cost:other}.}
        $\text{it} \gets 0, \text{UB} \gets +\infty, \text{LB} \gets -\infty$;\;
        \While{$\text{UB} - \text{LB} > \epsilon$}{
            $\text{it} \gets \text{it} + 1$\;
            Solve (Sub-MCP) to obtain $\text{z*, r*, R*}, \theta^*$.\;
            \uIf{$\max_{t,n}\{g^1_{tn}, g^2_{t}\} > 0$}{
                Add constraints \eqref{sub-MCP-Cost:cut-cons1} - \eqref{sub-MCP-Cost:cut-cons2} to (Sub-MCP).\;
                $\text{UB} \gets \theta^*$;\;
            }\Else{
                Add constraints \eqref{MCP-Cost:submodular1} - \eqref{MCP-Cost:submodular2} - \eqref{sub-MCP-Cost:cut-obj};\;
                $\text{UB} \gets \theta^*, \text{LB} \gets \max \{\text{LB}, \mathcal{F}(\text{z*,r*,R*})\}$;\;
            }
        }
        \Return \text{z*,r*,R*}.\;
\end{algorithm}

==> sections/5.Numerical_Experiments.tex <==
\section{Numerical Experiments}
\begin{align*}
V_{ti} &= \beta c_{ti}\\
U_{tn}^c &= e^{\beta\alpha b_{tn}}\\
U_t^c &= e^{\xi_t}
\end{align*}
